Event Transformer

The event camera's low power consumption and ability to capture microsecond brightness changes make it attractive for various computer vision tasks. Existing event representation methods typically convert events into frames, voxel grids, or spikes for deep neural networks (DNNs). However, these approaches often sacrifice temporal granularity or require specialized devices for processing. This work introduces a novel token-based event representation, where each event is considered a fundamental processing unit termed an event-token. This approach preserves the sequence's intricate spatiotemporal attributes at the event level. Moreover, we propose a Three-way Attention mechanism in the Event Transformer Block (ETB) to collaboratively construct temporal and spatial correlations between events. We compare our proposed token-based event representation extensively with other prevalent methods for object classification and optical flow estimation. The experimental results showcase its competitive performance while demanding minimal computational resources on standard devices. Our code is publicly accessible at \url{https://github.com/NJUVISION/EventTransformer}.

==> sections_full/approach.tex <==
\input{sections_full/figures/backbone}
\subsection{Problem Definition}
An event camera records a sequence of events asynchronously, which can be described in a mathematical form:
\begin{equation}\label{event}
    \mathbf{E }=\{{{e}_{i}}\}_{i=1}^{N},{{e}_{i}}=({{\vec{u}}_{i}},{{t}_{i}},{{p}_{i}})
\end{equation}
Each event $e_i$  independently includes a specific pixel position ${{\vec{u}}_{i}}=({{x}_{i}},{{y}_{i}})$ and polarity ${{p}_{i}}$ at a timestamp $t_i$. ${{p}_{i}}$ indicates the increase or decrease of pixel brightness. Equation \ref{event} reveals that the event stream is composed of asynchronous, sparse, and sub-uniformly distributed events, but the DNN cannot directly utilize this data format for downstream tasks. Therefore, this paper aims to create a backbone named Event Transformer to convert the raw event stream to a feature tensor with all the information of the original event fully preserved, which can be generalized to event-based vision tasks such as classification, segmentation and optical flow estimation.

\subsection{Spatiotemporal Encoding}
Essentially, a new event is triggered when the change in brightness $L$ of a pixel reaches a threshold $C$ (an intrinsic parameter of the event camera):
\begin{small}
    \begin{equation}
    \Delta L({{{\vec{u}}}_{i}},{{t}_{i}})=L({{{\vec{u}}}_{i}},{{t}_{i}})-L({{{\vec{u}}}_{i}},{{t}_{i-1}}) \ge {{p}_{i}}C,{{p}_{i}}\in \{-1,1\}  
\end{equation}
\end{small}
This implies that each event in the event stream is solely influenced by the change in brightness of the corresponding pixel itself between the previous timestamp and the current timestamp, independent of the brightness levels of other pixels at the exact timestamp or in previous instances. Consequently, a robust local temporal correlation is observed within the event stream. Furthermore, in accordance with the luminance invariance assumption and the motion consistency principle, the occurrence of events within a brief timeframe is exclusively attributed to the motion of objects within the visual field, establishing a close spatial relationship between each event and others within its neighboring spatial domain.
We devised a spatiotemporal encoding block to encompass temporal and spatial information to extract the temporal and spatial features from the unprocessed event stream. Initially, to separately encode the spatial features of the event stream, we compress the t-dimension and transform it into an event frame that fully retains all the information of the X/Y dimensions. Given the sparsity inherent in the event stream, only a minute percentage of the event frame contains valid pixel values. We employ sparse convolutional operations to enhance computational efficiency and extract pertinent features from the event frame. Subsequently, for encoding the temporal aspects of the event stream, we employ a multilayer perceptron (MLP) to process the timestamps of events with positive and negative polarity in a distinct manner. We consider polarity an inherent property that constitutes the essential condition for event triggering. Consequently, whether performing spatial or temporal encoding, the input data preserves the polarity information associated with the events. Finally, we concatenate the results obtained from spatial and temporal encoding and downscale them to a size of C-channel, utilizing an MLP, before feeding them as input to the subsequent EventTransformer Block. 

\subsection{Backbone Architecture}
In order to model the dependencies between events within an event stream and achieve efficient parallel processing of event data, we propose the EventTransformer block (ETB). Fig.~\ref{fig:et_backbone} depicts the Event Transformer backbone that consists of five ETBs to efficiently characterize the spatial-temporal correlations from input event sequence in a multistage means for output features.  As shown in Fig.~\ref{fig:et_block}, each ETB is formed by three-way attentions: local attention (LXAttn), sparse convolution attention (SCAttn), and global attention (GXAttn). 

At the first stage, raw event sequence $\bf E$ of size $\textit{N}\times 4$ is fed to the spatiotemporal encoding block to generate corresponding features $\bf F$ of size $N \times C$. It is noticed that original $\bf E$ is passed all the way through the Backbone used for position encoding and relation extraction. As a result, both events and associated features at a size of $N \times (4+C)$ are processed by the subsequent ETB. The output of the first stage is then processed by subsequent stages. Second to fifth stage introduce the {\it event merging} operation before the ETB. Each {\it event merging layer} is designed by a farthest point downsampling~\cite{pointnet++} step and a serious of layers including MLP-ReLU-BN, reducing the number of events uniformly by a factor of 4 and doubling the feature channel size. These steps eventually lead to a final output of size  $\frac{\textit{N}}{128}\times(32\textit{C}+4)$. In this work, $C$ is set to $32$ for the best balance between the computation cost and model effectiveness.

\input{sections_full/figures/ETB}
\subsection{Three-way Attention}
% \begin{figure}
% \centering
% % \includegraphics[width=0.96\textwidth]{figures/Local.pdf}
% \subfloat[Attention $s_{im}$ between $e_i$ and $e_m$]{\includegraphics[width=0.45\textwidth]{figures/Local_left.pdf} \label{fig:local_left}}\quad
% \subfloat[Self attention $s_i$ of $e_i$]{\includegraphics[width=0.45\textwidth]{figures/Local_right.pdf}\label{fig:local_right}}
% \caption{{\bf Self attention in LXformer.} {\bf (a)} The attention $s_{im}$ between $e_i$ and $e_m$ is calculated using query $q_i$ of $e_i$, key $k_m$ of $e_m$ and the distance $d_{im}$ between $e_i$ and $e_j$. {\bf (b)} The self-attention $s_i$ is calculated using the set $G_i$ of events that are temporally close to event $e_i$.}
% \label{fig:local_transformer}
% \end{figure}

In this section, we discuss details for the design of LXAttn, SCAttn, and GXAttn. 

\noindent {\bf Local Attention (LXAttn).} 
Since each event is triggered by a change in pixel brightness generated by coherent motion, adjacent events are interdependent in the temporal and spatial dimensions. To model the local spatiotemporal correlation between proximity events, we propose the LXAttn module. Let us consider an $N$-event sequence $\mathbf{E }=\{{{e}_{i}}\}_{i=1}^{N}\in {{\mathbb{R}}^{N\times 4}}$ as input for each LXAttn module. For each event $e_i$, we use KNN to find its nearest neighboring $k_l $ events ${{\mathbf{E }}_{KNN}}=\{{{e}_{j}}\}_{j=1}^{k_l }\in {{\mathbb{R}}^{k_l \times 4}}$ in the spatiotemporal dimension. To retain the position relationship between any two events like $e_i$ and $e_j$, we embed the relative spatiotemporal position using: 
\begin{equation}
    P{{E}_{loc}}({{e}_{i}},{{e}_{j}})=MLP(e_{i}^{xyt}-e_{j}^{xyt})\in {{\mathbb{R}}^{C'}}
\end{equation}
where $e_{i}^{xyt}$ represents the data of X-dimension, Y-dimension and t-dimension of the event $e_i$. The position embedding $P{{E}_{loc}}({{e}_{i}},{{e}_{j}})$ provides meaningful local relative spatiotemporal position information for the subsequent LXAttn calculation process. Moreover, the aggregated spatiotemporal features $\mathbf{F}\in {{\mathbb{R}}^{N\times C}}$ are fed into three different MLPs to derive the attention vectors $Q,K,V\in {{\mathbb{R}}^{N\times C'}}$. The self attention between $\boldsymbol{e}_i$ and its adjacent event $\boldsymbol{e}_{j} \in \mathbf{E}_{KNN}$ is computed as: 
\begin{small}
    \begin{equation}
        Attn_{ij}^{loc}={MLP({{q}_{{{e}_{i}}}}-{{k}_{{{e}_{j}}}}+P{{E}_{loc}}({{e}_{i}},{{e}_{j}}))}/{{{\sigma }_{loc}}}\;
    \end{equation}
\end{small}
where ${{\sigma }_{loc}}$is the const LXAttn attention scale. 
The local self attention $Attn_{i}^{loc}$ of $\boldsymbol{e}_i$ can be summed up by:
\begin{small}
    \begin{equation}
        Attn_{i}^{loc}=\sum{soft\max (Attn_{ij}^{loc})\odot ({{v}_{{{e}_{j}}}}+P{{E}_{loc}}({{e}_{i}},{{e}_{j}}))}
    \end{equation}
\end{small}
where ${{e}_{i}}\in \mathbf{E}$, ${{e}_{j}}\in {{\mathbf{E}}_{KNN}}$.

% The input of each LXAttn is an event sequence having $N$ events: $\mathbf{E} = \{\boldsymbol{e}_{1}, \ldots,\boldsymbol{e}_{N} \} \in \mathbb{R}^{N \times 4}$, with 4-channel attributes in each $\boldsymbol{e}_i$, and aggregated $C$-channel features $\mathbf{F} = \left\{ \boldsymbol{f}_{1}, \ldots, \boldsymbol{f}_{N} \right\} \in \mathbb{R}^{N \times \textit{C}}$. 
% We feed $\mathbf{F}$ into three different MLPs to derive the query, key, and value vectors of $\mathbb{R}^{ \textit{N}\times \textit{C}^\prime}$, denoted as $\mathbf{Q}$, $\mathbf{K}$, and $\mathbf{V}$, respectively. 
% In order to obtain the position relationship between any two events like $\boldsymbol{e}_i$ and $\boldsymbol{e}_j$, we encode the relative position by a MLP, noted as $\boldsymbol{pe}_{ij} = \textrm{MLP}\left( \boldsymbol{e}_i - \boldsymbol{e}_j \right), ~\boldsymbol{pe}_{ij} \in \mathbb{R}^{\textit{C}^{\prime}}$. When exploiting the local correlation of the event $\boldsymbol{e}_i$, we only consider $k_l$ events that are temporally closest to $e_i$ for pursuing computation efficient, and define them as a subset $\mathbf{E}_l$. 
% The self attention between $\boldsymbol{e}_i$ and its adjacent event $\boldsymbol{e}_{l} \in \mathbf{E}_l$ is computed as: 
% \begin{equation}
% \textit{local}_{il} = \textrm{MLP} \left( \boldsymbol{q}_i- \boldsymbol{k}_l + \boldsymbol{pe}_{il} \right). 
% \end{equation}
% The local self attention $\textit{local}_i$ of $\boldsymbol{e}_i$ can be summed up by:
% \begin{equation}
% \textit{local}_{i} = \sum\limits_{\boldsymbol{e}_{l} \in \mathbf{E}_l} \textrm{softmax}_l \left( \boldsymbol{s}_{il} \right) \odot \left( \boldsymbol{v}_{l}+\boldsymbol{pe}_{il} \right).
% \end{equation}

\noindent {\bf Sparse Convolution Attention (SCAttn).}
According to the trigger conditions of the event, the timestamps of the exact pixel locations closest to each other in the time dimension are correlated. However, in the spatial dimension, the spatial correlation of the nearest neighbor events at different pixel locations has uncertainty because the consecutive motion may come from arbitrary directions. In order to construct local correlations between events in the spatial dimension, we propose the SCAttn module. Firstly, we utilize the ball query algorithm to retrieve $k_{sc}$ events ${{\mathbf{E }}_{window}}=\{{{e}_{j}}\}_{j=1}^{k_{sc}}\in {{\mathbb{R}}^{k_{sc}\times 4}}$ within the 2D local window (e.g., 3×3 in this study) of each event and construct the position embedding by the relative position relationship between them: 
\begin{equation}
    P{{E}_{sc}}({{e}_{i}},{{e}_{j}})=MLP(e_{i}^{xy}-e_{j}^{xy})\in {{\mathbb{R}}^{C''}}
\end{equation}
Then, we stack features of all N events at the same spatial position for averaging and concatenating averaged features with two polarity panels (one accumulating positive events and one for negative). The sequence of events $\mathbf{E}$ is converted to a 2D event frame $\mathbf{I}\in {{\mathbb{R}}^{H\times W\times (2+C)}}$ with $H$ and $W$ as the height and width. Three different sparse convolutions obtain the query, key, and value vectors as :
\begin{small}
    \begin{equation}
        Q\text{ }=\text{ }SCon{{v}_{q}}\left( \mathbf{I} \right),
        K\text{ }=\text{ }SCon{{v}_{k}}\left( \mathbf{I} \right),
        V\text{ }=\text{ }SCon{{v}_{v}}\left( \mathbf{I} \right)
\end{equation}
\end{small}
Finally, similar to the LXAttn module, the local spatial self-attention $Attn_{i}^{sc}$ of $e_i$ can be written as:
\begin{small}
    \begin{align}
    & Attn_{i}^{sc}=\sum\limits_{{}}{soft\max (Attn_{ij}^{sc})\odot ({{v}_{{{e}_{j}}}}+P{{E}_{sc}}({{e}_{i}},{{e}_{j}}))} \\ 
        & \begin{matrix}
            & Attn_{ij}^{sc}=MLP({{q}_{{{e}_{i}}}}-{{k}_{{{e}_{j}}}}+P{{E}_{sc}}({{e}_{i}},{{e}_{j}}))/{{\sigma }_{sc}}\   \\
        \end{matrix} 
    \end{align}
\end{small}
where ${{\sigma }_{sc}}$is the const SCAttn attention scale, ${{e}_{i}}\in \mathbf{E}$, ${{e}_{j}}\in {{\mathbf{E}}_{window}}$.

% Different from the language data that only possesses the 1D dynamics over time,  events captured by the camera exhibit changes in both space and time. In addition to the local embedding using $k_l$ temporally-closest events in LXAttn to leverage the 1D time correlations, we suggest another local embedding in 2D space to exploit 2D spatial correlations. 

% To incorporate spatial correlations,  we first stack features of all events that occur at the same spatial position with the same polarity for averaging, and then concatenate averaged features for respective polarity levels. The sequence of events $\{(\boldsymbol{e}_i,\boldsymbol{f}_i)\}_{i=1}^N$ is converted to a 2D frame $\mathbf{I} \in \mathcal{R}^{\textit{H} \times \textit{W} \times \left(2+\textit{C}\right)}$, where $H$ and $W$ are the height and width of the frame.

% We extract the correlation between local 2D pixels in feature $\bf I$ through a sparse convolution-based attention mechanism. The attention query, key, and value vectors are obtained by three different sparse convolutions~\cite{sparse_conv} as $\mathbf{Q}= \textrm{SPConv}_q(\mathbf{I})$, $\mathbf{K}=\textrm{SPConv}_k(\mathbf{I})$, $\mathbf{V}=\textrm{SPConv}_v(\mathbf{I})$, and events located at the same pixel share the same $q$, $k$ and $v$. The use of sparse convolution is mainly due to the sparsely-scattered nature of events. 

% To reduce the computational complexity, for event $\boldsymbol{e}_i$, we retain its sparse-conv based self attention $\textit{sp}_i$ within its surrounding window $k_w$ (e.g., 3$\times$3 in this study) utilizing the similar attention calculation method as the $\textit{local}_i$ while the $\boldsymbol{pe}_{ij}$ is replaced by $\textrm{MLP}\left( \boldsymbol{u}_{i}-\boldsymbol{u}_{j} \right)$ since SCAttn is only designed for gathering the space information.

\noindent
{\bf Global Attention (GXAttn).}
LXAttn and SCAttn aggregate local features in both space and time dimensions. Specifically, LXAttn only allows the use of $k_l$ spatiotemporally-closest events, while the receptive field in SCformer is limited to the local window. However, for high-level vision tasks, the global relationship across all events is particularly important. If we directly enlarge the $k_l$ events in LXAttn to all events, the computational complexity will increase from $\textit{N}$ to $\textit{N}^2$, which is infeasible for large $N$. 

For the purpose of effectively processing and embedding global information, we down-sample the number of $\mathbf{E}$ from $N$ to $\hat{N}$, forming a subset $\mathbf{\hat{E}}$ and computing attention map with local $\mathbf{K}$ from original resolution and global $\mathbf{\hat{Q}}, \mathbf{\hat{V}}$ from $\mathbf{\hat{E}}$. More specifically, we first use the farthest point down-sampling with down-sample rate $k_r$ to select the most representative events $\mathbf{\hat{E}}$. For each $\boldsymbol{e}_g \in \mathbf{\hat{E}}$, its corresponding feature $\boldsymbol{\hat{f}}_g \in \mathbf{\hat{F}}$ is sampled from:
\begin{equation}
    \begin{split}
        \boldsymbol{\hat{f}}_g = \max_{\boldsymbol{e}_r \in \mathbf{E}_r} \left( {\rm MLP} \left( \textrm{Concat} \left( \boldsymbol{e}_r, \boldsymbol{f}_r \right) \right)  \right), 
    \end{split}
\end{equation}
where $\mathbf{E}_r$ is the set of
$\lfloor \frac{1}{\textit{r}} \rfloor$
nearest events of $e_g$. Then we derive $\mathbf{\hat{Q}}$ and $\mathbf{\hat{V}}$ from $\mathbf{\hat{F}}$. Afterwards, each event $\boldsymbol{e}_i$ is calculated the global self attention $\textit{global}_{i}$ with $k_l$ nearest events in $\mathbf{\hat{E}}$ with the same attention approach as $\textit{local}_i$. Finally, $\textit{local}_i$, $\textit{sp}_i$ and $\textit{global}_i$ are concatenated and fed into a MLP for the rest procedure in ETB.


==> sections_full/experiment.tex <==
In this section, we present our experiments to evaluate the classification, object detection and optical flow estimation performance of our proposed event transformer and existing methods. 

\subsection{Event-based Classification}
% \def\nmnist{$\textbf{N}$$\mhyphen$$\textbf{MNIST}$}
% \def\snmnist{$\textbf{N}$$\mhyphen$$\textbf{M}$}
% \def\ncaltech{$\textbf{N}$$\mhyphen$$\textbf{Caltech101}$}
% \def\sncaltech{$\textbf{N}$$\mhyphen$$\textbf{Cal}$}
% \def\cifar{$\textbf{CIFAR10}$$\mhyphen$$\textbf{DVS}$}
% \def\scifar{$\textbf{CIF10}$}
% \def\ncars{$\textbf{N}$-$\textbf{Cars}$}
% \def\sncars{$\textbf{N}$$\mhyphen$$\textbf{C}$}
% \def\asl{$\textbf{ASL}$$\mhyphen$$\textbf{DVS}$}
% \def\sasl{$\textbf{ASL}$}
\def\nmnist{N-MNIST}
\def\snmnist{N-M}
\def\ncaltech{N-Caltech101}
\def\sncaltech{N-Cal}
\def\cifar{CIFAR10-DVS}
\def\scifar{CIF10}
\def\ncars{N-Cars}
\def\sncars{N-C}
\def\asl{ASL-DVS}
\def\sasl{ASL}


\noindent \textbf{Datasets and metric} We test our model on five event-based classification datasets: \nmnist~\cite{nMnist}, \ncaltech~\cite{n_caltech101},  \cifar~\cite{cifar10_dvs}, \ncars~\cite{nCars} and \asl~\cite{asl_dvs}. As shown in Table.~\ref{table:cls_datasets_compare}, these datasets vary significantly in terms of captured camera, source of events, average duration of event stream, and dataset size. \nmnist, \ncaltech\ and \cifar\ were shot with a laboratory version of event camera (Asynchronous Time-based Image Sensor Lab Sensor). The data capture equipment consists of an e-link screen, a movable tripod head, and an event camera. Images from the existing MNIST~\cite{lecun2013mnist}, Caltech101~\cite{fei2004learning} and CIFAR-10~\cite{krizhevsky2009learning} are displayed on the monitor and the tripod head for the event camera is moved to generate events. Since the e-link screen does not refresh while the content remains unchanged, noisy events due to screen refresh are avoided. These events arise due to camera shake, which is  different from events generated by motion in the real world. \ncars\ used the event camera (Prophesee Gen1) to record 24,029 sequences of 100ms on the city roads, and split them into cars and background. \asl\ is a 24-class dataset of  handshape recordings under realistic conditions using DAVIS240c. Compared to the previous datasets, \asl\ has ten times more event sequences.
We train our model on the training set of each dataset separately and evaluate the Top-1 classification accuracy on the test set. For datasets (\ncaltech, \cifar\ and \asl) without official division between training and test sets, we follow the setup introduced in ~\cite{asl_dvs,EV-VGCNN,xie2022vmv} and randomly sample 80\% of the data for training and the remaining 20\% for testing.

\input{sections_full/tables/classification_dataset}

\noindent \textbf{Implementation details}
For the classification task, we average the stage 4 output features of all events and feed them into a classification head consisting of layer normalization and linear regression to get the final output category. 
The number of channels $C$ for stage 1 is set to 32. The interactive events $k_l$ in LXAttn and GXAttn is set to 16. The size of window $k_w$ in SCAttn is set to 3. And the farthest down-sampleing rate $r$ in GXAttn is set to $32, 32, 16, 8, 4$ in each stage separately. At training time, 2048 events are randomly sampled from the training set as input without any augmentation tricks, and all events are input during inference. We train our model from scratch for 200 epochs by optimizing the cross-entropy loss using the SGD optimizer with momentum 0.9 and the batch size of 64. The learning rate starts from 0.01 and decays to 0.001 and 0.0001 at 150 and 180 epochs, respectively. The whole training process takes only a few hours (e.g., only three hours for \ncaltech).
\input{sections_full/tables/classification_results}

\noindent \textbf{Experimental results}
We compare Top-1 classification accuracy obtained from our model with frame-based methods~\cite{hfirst, hots, nCars, EST, AMAE, M-LSTM, MVF-Net, he2016deep}, voxel-based methods~\cite{Eventnet, asl_dvs, EV-VGCNN, xie2022vmv} and spike-based methods~\cite{gabor_snn, PLIF}. 
%
The models in EST~\cite{EST}, M-LSTM~\cite{M-LSTM} and MVF-Net~\cite{MVF-Net} were pretrained using ImageNet~\cite{krizhevsky2012imagenet}; thus for a fair comparison, we used the results from ~\cite{xie2022vmv} that trains networks from scratch. For PLIF~\cite{PLIF}, the original paper divides the dataset into 9:1 for training and testing; therefore, we report the results by retraining their model with 80/20\% train/test split using their official code. As shown in Table~\ref{table:classification_results}, our model achieves state-of-the-art results on all of the classification datasets which illustrates the effectiveness of our model and representation form.
We also compare the number of parameters (Parameters), the floating point operations (FLOPs), and the final accuracy of different methods on the \ncaltech\ dataset using the same calculation method in ~\cite{xie2022vmv, EV-VGCNN}.  The computation cost of~\cite{hfirst,hots,nMnist} are not listed since they are not neural-network based methods. For the spike-based methods~\cite{gabor_snn,PLIF}, the FLOPs is measured under common environments (CPU and GPU) since they require special hardware devices for their inference. We get the best performance using the least amount of computation (only 0.51G FLOPs). Thus, our proposed event transformer is suitable for low-power devices in conjunction with event camera, where the computational cost is the primary concern.

\subsection{Event-based Object Detection}
\noindent \textbf{Datasets and metric} Event-based object detection is designed for regress the object bounding boxes within event stream under different scenarios, especially under the low-light and high-speed condition. Following previous papers~\cite{aegnn,nvs-s}, we evaluate our model on two challenging datasets, N-Caltech101~\cite{n_caltech101} and Gen1~\cite{gen1}. N-Caltech101~\cite{n_caltech101} is the very first events detection dataset having one bounding box for each event sequence. While the Gen1~\cite{gen1} dataset extremely extends the number of the data with 255781 bounding boxes for cars and pedestrians captured under autonomous driving scenes. For measuring performance, we use the eleven-point mean average precision (mAP)~\cite{coco} score.

\noindent \textbf{Implementation details}
Similar to the previous work~\cite{aegnn, yole, asynet, nvs-s}, we adopt a YOLO-based detection head~\cite{yolo} implemented by ~\cite{mmdetection}. The backbone setting is as same as the one we used in classification tasks. We train the detector from scratch for 300 epochs with the batch size of 64 optimized by SGD. The learning rate starts from 0.01 and decreases to 0.0001 linearly. It cost one day for the entire training.

\noindent \textbf{Experimental results}
\input{sections_full/tables/detection_results}
The comparison results is shown in Table.~\ref{table:detection_results}. Our method achieves minimization computation cost ($540\times$ lower on N-Caltech101~\cite{n_caltech101} dataset and $20000\times$ lower on Gen1~\cite{gen1} dataset) compared with previous SOTA methods. While Asynet~\cite{asynet} has better accuracy on N-Caltech101~\cite{n_caltech101} dataset, our model outperforms 8.9 mAP on Gen1~\cite{gen1} dataset since ~\cite{asynet} is designed with the prior detecting only single object in a event sequence. Conductive to the dense, synchronous recurrent network, RED~\cite{1Mdetection} achieves best performance on Gen1~\cite{gen1} dataset while needs 4712 MFLOP to calculate a single event.

\subsection{Event-based Optical Flow Estimation}
\noindent \textbf{Dataset and Metrics}
We use the MVSEC dataset~\cite{mvsec} dataset captured in both indoor flying and outdoor driving scenarios using stereo event cameras for training and evaluation. The ground truth labels of optical flow are estimated by depth and IMUs. Although the indoor data is as different again from the outdoor, we only use the outdoor\_day2 sequence for training and rest parts for testing following the basic settings in ~\cite{spike-evflownet}.
Average End-point Error (AEE) and Outlier AEE larger than three pixel  (OUT) are set as the evaluation metrics keeping same as the ~\cite{ev_flownet, spike-evflownet}.
Considering the sparse nature of events, both AEE and OUT are only counted in terms of activated pixels. We compute the AEE and OUT for $dt=1$ (about \SI{22}{\milli\second}) since longer interval (e.g.\ $dt=4$) does not cohere with the low-delay characteristic of the event camera. 

\noindent \textbf{Implementation details}
We first adopt the U-Net~\cite{unet} based encoder-decoder architecture to estimate the moving speed of every event. And then we derive the optical flow by multiple time $t$ to event speeds. The archtecure of the encoder is similar to the backbone used in our classification model besides the down-sample rate in {\it event merging layer} of stage two is set to two preventing losing too much details.
During training, we optimize our model with SGD optimizer for 25000 iterations and the leanrning rate is set to 0.005 decayed by 0.1 at 15000 and 20000 iterations. The training input is 4096 random sampled events with batch size of 12, whereas all events are fed in at the inference period. We choose Charbonnier loss~\cite{Charbonnier-loss}, a common loss in the optical flow literatures~\cite{Charbonnier-loss,ev_flownet},as loss function.

\noindent \textbf{Experiment results}
\input{sections_full/tables/optical_flow_results}
We provide quantitative evaluations in Table.~\ref{table:optical_flow_results}. All of the sequences are center cropped of $256\times256$ and we use all data in indoor\_flying scene but only 800 sequences for the outdoor\_day1 sequence keeping same as ~\cite{ev_flownet, spike-evflownet}. As provided in ~\cite{shiba2022secrets}, different loss functions lead to significant difference testing results. Thus we retrain the FireNet~\cite{firenet}, LIF-EvFlowNet~\cite{spike-evflownet} and LIF-FireNet~\cite{spike-evflownet} utilizing the official provided code within the same loss function as ours and EV-FlowNet~\cite{ev_flownet} for fair comparison.
Overall, our model outperforms in terms of AEE on all sequences using only 39\% computation cost.

\subsection{Ablation Study}
We conduct a number of experiments with various setting of our model as an ablation study on \cifar. First we analyze the efficiency of our LXAttn, SCAttn, and GXAttn. Then we analyze the effect of the number of interactive events $k_l$ in LXAttn and window size $k_w$ in SCAttn.

\noindent \textbf{Network structure.} We demonstrate that each part of our network is essential through several sets of  experiments. Table~\ref{table:ablation_structure} shows different components of the network structure, where L, S, and G represent LXformer, SCformer and GXformer, respectively. For the comparision of Local and Local+Sparse, we found that the addition of SCformer significantly improved the model's representation ability (+1.8). Local+Sparse+Global shows that the addition of GXformer can further aggregate global information and improve performance (+1.2). We also experimented with the placement of LXformer, SCformer, and GXformer (Global+Local+Sparse and Local+Sparse+Global), and the experimental results showed that premature aggregation of spatial and global information is not conducive to the model performance (-1.4 and -1.6). We believe that this is due to the fact that temporal relationship is the most fundamental property for event data.
% The comparison of Local and Local (Duplicate), and Local+Sparse and Local+Sparse (Duplicate), shows that simply adding duplicate modules does not improve the model performance significantly. However, the comparison between Local and Local+Sparse and between Local+Sparse and Local+Sparse+Global  shows that the addition of both SCformer and GXformer effectively improves the performance of the model by +1.8 and +1.2 points. 
% \Salnote{I did not fully understand what is changing in this ablation study.} 
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Ablation Study of Network Structure}
\label{table:ablation_structure}
\begin{tabular}{llc}
\toprule\noalign{\smallskip}
\textbf{Type} & \textbf{Structure} & \textbf{Top-1 Accuracy} \\
\noalign{\smallskip}
\midrule
\noalign{\smallskip}
Local & \text{[L, L, L, L]} &  68.2 \\
Local+Sparse & \text{[LS, LS, LS, L]} & 70.0 \\
Sparse+Local+Global & \text{[SL, SLG, SLG, L]} & 69.8 \\
Global+Local+Sparse & \text{[LS, GLS, GLS, L]} & 69.6 \\
\textbf{Local+Sparse+Global} & \textbf{[LS, LSG, LSG, L]} & \textbf{71.2} \\
\bottomrule
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

\noindent \textbf{Fusion of LXformer and SCformer.}
The LXformer extracts temporal features, while the SCformer extracts spatial features. We conducted a series of experiments to find the best way to fuse the two sets of features. Table~\ref{table:ablation_fusion} presents results when we try to fuse the features in three ways: Concatenate, Parallel, and Serial. 
%
In Concatenate setting, we try to connect two completely different features together by concatenating them, and then adding them to the input features after reducing their dimension using an MLP. As shown in the Table~\ref{table:ablation_fusion}, this will have an adverse impact on the model performance (-9.2). We believe this is because of the lack of residual connection between input features and output features both in LXformer and SCformer, which is important for transormers. Then we compared the performance of connecting the two features in parallel and series. The experimental results show that the temporal information aggregated by LXformer can help SCformer to extract the spatial information when using serial fusion (+1.2). Therefore we chose to place the SCformer module after the LXformer module in our proposed model.

\setlength{\tabcolsep}{4pt}
\begin{table}[t]
\begin{center}
\caption{Ablation Study of Fusion of LXformer and SCformer}
\label{table:ablation_fusion}
\begin{threeparttable}
9\begin{tabular}{lcc}
\toprule\noalign{\smallskip}
\textbf{Type} & \textbf{Combination\tnote{$\dagger$}} & \textbf{Top-1 Accuracy} \\
\noalign{\smallskip}
\midrule
\noalign{\smallskip}
Concatenate & Y = X + {\rm MLP}({\rm Concat}(L(X)+S(X))) & 62.0 \\
Parallel & Y = X + L(X)+S(X) & 70.0   \\
\textbf{Serial} & \textbf{Y = X + S(X+L(X))} &  \textbf{71.2} \\
\bottomrule
\end{tabular}
\begin{tablenotes}
    \footnotesize
    \item[$\dagger$] Symbol definition: X is the input features, Y is the output, L is the LXformer and S is the SCformer.
    \end{tablenotes}
\end{threeparttable}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

\noindent \textbf{Number of closest events in LXformer.}
In LXformer, we interact each event with $M$ events that occur adjacent to it in the temporal sequence, and here we experiment with the number of closeest events. Table~\ref{table:ablation_lxformer} shows that when the number of closest events is small ($M=4$ or $M=8$), LXformer cannot extract enough content information (the performance drops -5.4 and -1.2, respectively). When the number is very large ($M=32$ or $M=64$), it introduces too many noisy events and causes a loss of attention (the performance drops -0.3 and -1.6, respectively). 

% \Salnote{What is the main takeaway of these results?} 
% \Salnote{Also, I do not remember where you discussed $M$ in the description of the technical approach.} 


\setlength{\tabcolsep}{4pt}
\begin{table}[]
\begin{center}
\caption{Ablation Study of Closest Events in LXformer}
\label{table:ablation_lxformer}
\begin{tabular}{lccccc}
\toprule\noalign{\smallskip}
\textbf{$M$ Closest Events in LXformer} & 4 & 8 & \textbf{16} & 32 & 64 \\
\noalign{\smallskip}
\midrule
\noalign{\smallskip}
\textbf{Top-1 Accuracy} & 65.8 & 69.0 & \textbf{71.2} & 70.9 & 69.6 \\
\bottomrule
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

\noindent \textbf{Size of interactive window in SCformer.}
In SCformer, we compute self attention for each event in the frame plane for a window size of $W$. Therefore, we experimented with the size of the window $W$. The experimental results shown in Table~\ref{table:ablation_scformer} illustrate that if the window size is $1\times1$, the self attention degenerates to a general conv. The best results are achieved when the window size is $3\times3$. And when the window size is further increased, it does not bring better gain.

i\setlength{\tabcolsep}{4pt}
\begin{table}[]
\begin{center}
\caption{Ablation Study of Window Size in SCformer}
\label{table:ablation_scformer}
\begin{tabular}{lccccc}
\toprule\noalign{\smallskip}
\textbf{Size of $W$ in SCformer} & $1\times1$ & \textbf{$3\times3$} & $5\times5$ & $7\times7$ & $9\times9$ \\
\noalign{\smallskip}
\midrule
\noalign{\smallskip}
\textbf{Top-1 Accuracy} & 69.9 & \textbf{71.2} & 71.1 & 71.0 & 70.6 \\
\bottomrule
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

\noindent \textbf{Down-sample rate in GXformer.}
Finally, we evaluated the impact of down-sampling rate $r$ in GXformer on the model performance. As shown in Table~\ref{table:ablation_gxformer}, when the down-sampling rate $r$ is 1, which means no down-sampling, GXformer degenerates to LXformer. The experimental results show that when the $r$ is small (1 and 8), the global information extracted is not comprehensive (-1.4 and -0.9). And when the $r$ is too larger (64 and 128), it leads to excessive information loss (-0.6 and -1.1). Therefore we finally choose a downsampling rate of 32.

\setlength{\tabcolsep}{4pt}
\begin{table}[]
\begin{center}
\caption{Ablation Study of Down-sample Rate in GXformer}
\label{table:ablation_gxformer}
\begin{tabular}{lccccc}
\toprule\noalign{\smallskip}
\textbf{Down-sample rate $\textit{r}$ in GXformer} & 1 & 8 & \textbf{32} & 64 & 128 \\
\noalign{\smallskip}
\midrule
\noalign{\smallskip}
\textbf{Top-1 Accuracy} & 69.8 & 70.3 & \textbf{71.2} & 70.6 & 70.1 \\
\bottomrule
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

==> sections_full/figures/ETB.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.81\textwidth]{figures/ETB.pdf}
\label{fig:etb}
\caption{{\bf Event Transformer.} \textbf{(a)} Four-stage backbone with $N\times4$ raw events input and $\frac{N}{128}\times(32C+4)$ output. For each event, output includes the original 4-channel attributes and aggregated features. 
For simplicity, we only give the size of features at each stage. Linear embedding layer that uses a MLP is used at the 1st stage to map input 4-channel attributes of event to $C$-channel latent features for subsequent processing. From the 2nd to 5th stage, an event merging layer with a farthest point downsampling and a MLP-ReLU-BN is included before the ETB step. \textbf{(b)} the Event Transformer Block (ETB) consist of three parallel attentions. Local Attention (LXAttn), sparse convolution-based attention (SPAttn), global attention (GXAttn), and layer normalization (LN Norm) are standard layers from transformers.}
\label{fig:etb}
\end{figure*}


==> sections_full/figures/backbone.tex <==
\begin{figure*}[t]
\centering
\subfloat[Event Transformer Backbone]{\includegraphics[width=0.81\textwidth]{figures/backbone0.pdf}
\label{fig:et_backbone}}
\subfloat[Event Transformer Block]{\includegraphics[width=0.18\textwidth]{figures/backbone1.pdf}
\label{fig:et_block}}
\caption{{\bf Event Transformer.} \textbf{(a)} Four-stage backbone with $N\times4$ raw events input and $\frac{N}{128}\times(32C+4)$ output. For each event, output includes the original 4-channel attributes and aggregated features. 
For simplicity, we only give the size of features at each stage. Linear embedding layer that uses a MLP is used at the 1st stage to map input 4-channel attributes of event to $C$-channel latent features for subsequent processing. From the 2nd to 5th stage, an event merging layer with a farthest point downsampling and a MLP-ReLU-BN is included before the ETB step. \textbf{(b)} the Event Transformer Block (ETB) consist of three parallel attentions. Local Attention (LXAttn), sparse convolution-based attention (SPAttn), global attention (GXAttn), and layer normalization (LN Norm) are standard layers from transformers.}
\label{fig:network}
\end{figure*}


==> sections_full/figures/cover.tex <==
\begin{figure*}[t]
\centering
\subfloat[Representation Forms]{\includegraphics[width=0.23\textwidth]{figures/cover_0.pdf}
\label{fig:representation_forms}}\quad
\subfloat[Classification Gain]{\includegraphics[width=0.23\textwidth]{figures/cover_1.pdf}
\label{fig:classification_gain}}\quad
\subfloat[Detection Gain]{\includegraphics[width=0.23\textwidth]{figures/cover_2.pdf}
\label{fig:detection_gain}}\quad
\subfloat[Optical Flow Estimation Gain]{\includegraphics[width=0.23\textwidth]{figures/cover_3.pdf}
\label{fig:optical_flow_gain}}
\caption{\textbf{Our data representation forms and gain.} \textbf{(a)} Different representation forms of event data. The frame-based loses the temporal information, the voxel-based lacks temporal fine-grained, the spike-based cannot be effectively optimized due to non-differentiable of impulse response function and our proposed representation treats events as a sequence of discrete tokens with image properties which can utilize the temporal information of event data and its image nature while ensuring the lossless time precision. \textbf{(b-d)} Our Event Transformer outperforms existing state of the arts while maintaining efficiency.}
\label{fig:forms_and_gain}
\end{figure*}


==> sections_full/introduction.tex <==
\input{sections_full/figures/cover}
\label{sec:intro}
In contrast to a conventional camera that outputs standard intensity frame at fixed time interval, an event camera mimics the biological behavior of the retina~\cite{first_dvs_hardware_paper} to dynamically and asynchronously capture the intensity change of a pixel whenever it is beyond a preset threshold. As extensively reviewed in ~\cite{survey}, an event camera typically has a much higher response frequency (\SI{1}{\micro\second} vs \SI{33}{\milli\second}), lower power consumption (\SI{10}{\milli\watt} vs \SI{300}{\milli\watt}), and higher dynamic range (\SI{140}{\dB} vs \SI{70}{dB}). These advantages have led to the widespread use of event cameras in various computer vision tasks including object classification~\cite{nMnist,mnist_dvs,n_caltech101,cifar10_dvs,nCars,asl_dvs}, detection~\cite{1Mdetection, n_caltech101}, and optical flow estimation~\cite{mvsec,mvsec_optical_labels}.
% simultaneous localization and mapping (SLAM) \cite{slam1,slam2}.

An event camera records a sequence of events asynchronously, which can be described as 
\begin{equation}
    \mathbf{E}=\left\{\boldsymbol{e}_{1}, \boldsymbol{e}_{2}, \ldots, \boldsymbol{e}_{n}\right\}, ~\boldsymbol{e}_i = (\vec{u}_i, t_i, p_i).
  \label{eq:events_formulation}
\end{equation}
Each event $\boldsymbol{e}_i$ is a tuple that has pixel position $\vec{u}_i = (x_i, y_i)$, polarity $p_i \in \{-1, 1\}$ at time $t_i$.
$p_i$ indicates the increase or decrease of pixel brightness. To facilitate the use of event camera in downstream tasks, we first need to represent the events appropriately. 

Fig.~\ref{fig:representation_forms} depicts some common representation schemes that include frame-based~\cite{hfirst, hots, nCars, EST, AMAE, M-LSTM, MVF-Net, asynet, yole, ev_flownet, firenet}, voxel-based~\cite{Eventnet, asl_dvs, EV-VGCNN, nvs-s, aegnn}, and spike-based~\cite{gabor_snn, PLIF, spike-evflownet} representations. 

Instead of processing every pixel of the stacked plane wastefully, in this work, we propose to directly process the event sequence $\mathbf{E}$ in its native {\it vectorized tensor} format as a sequence of \textit{event words}. 
We observe that each events $\boldsymbol{e}_i = (\vec{u}_i, t_i, p_i)$ can be viewed and represented as a word in an event sequence, akin to representation of a word in a sentence for natural language processing (NLP) applications. Different parameters for the event $(\vec{u}_i, t_i, p_i)$ correspond to different words in a sentence. Note that a sentence in NLP tasks only presents word dynamics over time. In contrast, events occur sparsely over 2D space and asynchronously over time, which requires a representation that can preserve the joint spatiotemporal correlations. 

This work proposes a novel Event Transformer to  process the sequence of events ${\bf E}$ directly without event accumulation (e.g., averaging) to form a 2D frame, 3D voxel, or 2D spikes. To achieve this goal, we introduce a basic Event Transformer Block (ETB) that consists of three-way attention mechanism:  local attention (LXAttn), sparse-conv attention (SCAttn), and global attention (GXAttn). The LXAttn runs within a local 1D time duration to capture temporal correlations, the SCAttn performs the spatial information embedding in a predefined 2D local spatial window, and the GXAttn aggregates the information of downscaled sequence from the previous stage in a global manner. 

We concatenate five ETBs to create the event transformer backbone to convert input event stream to a feature tensor. Our goal is to extensively exploit spatial and temporal correlations of input event sequence by local and global information processing and generate effective spatiotemporal features for downstream tasks. Different from spike-based method, our method can be easily implemented on mainstream devices since we only use common operators like multilayer perceptron (MLP) and sparse convolution. Attention components in each ETB also offer computational efficiency; for instance the GXAttn runs on downscaled sequence of event features that can be achieved with local computations over segments of the event sequence.

We evaluate the proposed Event Transformer both high-level event-based classification and object detection tasks, and low-level optical flow estimation. We conducted extensive experimental studies to compare our proposed method with \zhihao{twenty (revise this number)} existing models that use frame-based, voxel-based, and spike-based representation. First, as shown in Fig.~\ref{fig:classification_gain}, we obtained the state-of-the-arts (SOTA) results for 
% N-MNIST~\cite{nMnist} (+0.4), N-Caltech101~\cite{n_caltech101} (+1.1), CIFAR10-DVS~\cite{cifar10_dvs} (+1.9), N-CARS~\cite{nCars} (+0.1), and ASL-DVS~\cite{asl_dvs} (+1.0) 
classification datasets (+0.1~1.9) 
% respectively
while reducing the amont of computational (-61\%) significantly compared with the previous SOTA. Next, conducive to processing event by event, we achieve 30000x computation efficient than the previous dense and synchronous recurrent detection network~\cite{asynet} given in Fig.~\ref{fig:detection_gain}. At last, within 3.5G FLOPs (-70\%), our Event Transformer produces more accurate optical flow especially on outdoor\_day1 sequence (AEE -0.12, OUT -1.16) illustrated in Fig.~\ref{fig:optical_flow_gain}.
Our method also requires the least computational resources compared to the existing methods, which makes it a practical and useful candidate for event-based vision tasks.

The main contributions of this paper are summarized as follows.
\begin{itemize}
    \item We propose a novel representation form {\it vectorized tensor} that takes full advantage of the image properties of the event while maintaining the fine-grained timestamps of the event.
    \item We propose the Event Transformer using {\it vectorized tensor} to fully extract the relationship between event and event.
    \item We achieve the highest accuracy on multiple datasets (including high-level and low-level) while also significantly reducing model computation.
\end{itemize}


==> sections_full/related_work.tex <==
\zhihao{should we remove the related work like the previous events paper in ICASSP~\url{https://ieeexplore.ieee.org/document/9747018}}
\subsection{Event Representation Methods}
Given the popularity and prevalence of deep neural network (DNN) for 2D images, it is attractive to re-use them for event cameras. 
A straightforward approach is to convert event sequence into a 2D image by aggregating events in a preset time duration (e.g., \SI{33}{\milli\second}) into a gray-scale frame, as shown in Fig.~\ref{fig:representation_forms}. A number of such frame-based event representation approaches have been proposed in \cite{hfirst, hots, nCars, EST, AMAE, M-LSTM, MVF-Net, asynet, yole, ev_flownet, firenet}, but they introduces motion blur by discarding the fine time granularity in event cameras. 
An alternative approach is to convert events into a 3D point cloud and apply 3D DNNs for different tasks. 
Voxel-based representation~\cite{Eventnet, asl_dvs, EV-VGCNN, nvs-s, aegnn} converts events into a sequence of spatially-scattered 3D voxels by aggregating events in a relatively-short time duration.
Some methods~\cite{gabor_snn, PLIF, spike-evflownet} represent events as impulses, as demonstrated in Fig~\ref{fig:representation_forms}, which resemble spikes in human brain neurons and try to process them with the spiking neural network (SNN), 
Nevertheless, a spike in SNN is an impulse response function which is not differentiable. Thus, the inability of SNN to usegradient-based backpropagation and the need for specialized hardware implementation limit its applications. 

\subsection{Event-Based Vision}
Event cameras were first used in SLAM because of their low latency and bandwidth savings compared to conventional video cameras. In SLAM, the most common vision task is the detection of calibration plates and feature points. Therefore, several methods proposed to detect corners, lines, and edges by manually designing feature extractors \cite{corner_1,corner_2,corner_3}. As event cameras are upgraded and popularized, they are increasingly used in tasks such as object recognition~\cite{nMnist,n_caltech101,cifar10_dvs,nCars,asl_dvs} and detection~\cite{1Mdetection,n_caltech101}. Extracting semantic information from purely hand-designed features is extremely difficult; therefore, several methods have converted events into images to extract features with DNNs~\cite{ev_meet_dl,ev_flownet,hfirst,hots,EST,AMAE,M-LSTM,MVF-Net}. For instance, \cite{ev_meet_dl} stacks a period of events into a two-channel image based on their polarity, which causes a loss of temporal information and the event data converts into a long-exposure photograph. \cite{ev_flownet} adds two channels to record the timestamp of the last event. To take full advantage of the temporal information, \cite{nCars} encodes the latest events into time-surfaces, but it loses the spatial features. \cite{EST,M-LSTM} attempt to generate event frames by adaptive selection of events using learning approaches. It is worth noting that all frame-based methods require selection of a time window. A shorter window leads to insufficient accumulated data for downstream tasks, while a longer one causes motion blur and defeats the original purpose of high response rate from event cameras.

Several methods have been introduced to represent and exploit the spatio-temporal correlations in the event data by processing them as 3D points ~\cite{asl_dvs,EV-VGCNN}. For instance. \cite{asl_dvs,EV-VGCNN,aegnn} use graph convolution network (GCN) to learn the relationship between down-sampled events because event data are extremely sparse and dense convolutions can be computationally intensive. The time required to build the graph structure can even exceed the time required for the recognition task itself. Furthermore, these methods pre-process data by voxelizing events, which reduces the temporal granularity of the event data.

In addition to DNN and GNN, some methods \cite{gabor_snn, PLIF, spike-evflownet} have used spiking neural networks (SNN) for event data processing. The design of SNNs simulating human neural response and event cameras simulating retinal activation appear to be a nice combination. Nevertheless, the challenges of training SNNs and the need for special hardware prevents SNN from being used in real-life applications \cite{tavanaei2019deep}. 

In summary, the current methods for processing of events face problems in combining the spatial and temporal information and preserving the fine temporal granularity. In our method, we use the raw events data as input to ensure the lossless time precision. Inspired by recent NLP literature ~\cite{bert,xlnet,transformer-xl}, we use a transformer to extract temporal features and fuse temporal features with spatial features by sparse convolutions.

\subsection{Transformer}
Transformer architecture was recently proposed in \cite{attention_is_all_u_need} and applied to machine translation, which contains self-attention layers without any recurrent or convolution blocks. In recent years, transformer-based methods have achieved huge success in NLP~\cite{bert,xlnet,transformer-xl} and vision tasks~\cite{vit,swin}. Transformer-based backbones achieve better performance compared to the convolution-based backbones because of their ability to model information over long duration. Recently, \cite{neimark2021video} has used video transformer to successfully process spatio-temporal information in videos. 
Recently, \cite{event_transformer_frame,event_transformer_video} have a trial to introduce transformer~\cite{vit} into event data by stacking events into frame losing time granularity.   
The NLP transformers~\cite{attention_is_all_u_need,bert,xlnet,transformer-xl} cannot consider the spatial information of events data, the image transformers cannot handle the temporal relationships of events, and the video transformer~\cite{neimark2021video} needs to voxelize events where the sparsity of events would result in a lot of redundant computations.
% Most related to our work is the Point Transformer\cite{point_transformer}. It suggest that point clouds are sets with semantic information that are non-uniformly distributed in space and are well suited for establishing intrinsic connections using the attention mechanism. 
% \Salnote{What is the most relevant transformer work? Why don't we discuss this point transformer?} 



==> sections_full/tables/classification_dataset.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table}
\begin{center}
\caption{List of Event-based Classifiaction Datasets}
\label{table:cls_datasets_compare}
\begin{threeparttable}
\begin{tabular}{lrrrr}
\toprule\noalign{\smallskip}
\textbf{Dataset} & \textbf{Camera} & \textbf{Source}\tnote{$\dagger$} & \textbf{Classes} \\
\noalign{\smallskip}
\midrule
\noalign{\smallskip}
\nmnist~\cite{nMnist} & ATIS Lab Sensor & shake cam  & 10 \\
\ncaltech~\cite{n_caltech101} & ATIS Lab Sensor  & shake cam & 101 \\
\cifar~\cite{cifar10_dvs} & ATIS Lab Sensor & shake cam & 10 \\
\ncars~\cite{nCars} & Profhesee Gen1 & real move & 2 \\
\asl~\cite{asl_dvs} & DAVIS240c  & real move & 24 \\
\bottomrule
\end{tabular}
\begin{tablenotes}
    \footnotesize
    \item[$\dagger$] Source of generating events.
    % \item[$\ddagger$] Average duration of event stream.
    \end{tablenotes}
\end{threeparttable}
\end{center}
\end{table}


==> sections_full/tables/classification_results.tex <==
\setlength{\tabcolsep}{3.8pt}
\begin{table*}[t]
\begin{center}
\caption{Accuracy of Event-based Classification Using Various Datasets. \snmnist\ refers to \nmnist, \sncaltech\ to \ncaltech, \scifar\ to \cifar, \sncars\ to \ncars, and \sasl\ to \asl.}
\label{table:classification_results}
\begin{tabular}{lrrrccccc}
\toprule\noalign{\smallskip}
\textbf{Method}   & \textbf{Representation} & \textbf{Parameters (M)} & \textbf{FLOPs (G)} & \textbf{\snmnist}~\cite{nMnist} & \textbf{\sncaltech}~\cite{n_caltech101} & \textbf{\scifar}~\cite{cifar10_dvs} & \textbf{\sncars}~\cite{nCars} & \textbf{\sasl}~\cite{asl_dvs} \\
\noalign{\smallskip}
\midrule
\noalign{\smallskip}
H-First~\cite{hfirst}           & frame & - & -   & 0.712        & 0.054                 & 0.077                & 0.561           & -                \\
HOTS~\cite{hots}              & frame  & - & -  & 0.808            & 0.210                  & 0.271                & 0.624           & -                \\
HATS~\cite{nCars}              & frame & - & -  & 0.991            & 0.642                 & 0.524                & 0.902           & -                \\
EST~\cite{EST}               & frame & 21.38 & 4.28 & 0.990            & 0.753                 & 0.634                & 0.919           & 0.979            \\
AMAE~\cite{AMAE}              & frame & 21.80 & 7.36 & 0.983            & 0.694                 & 0.620                & 0.936           & 0.984            \\
M-LSTM~\cite{M-LSTM}            & frame & 21.43 & 4.82  & 0.986            & 0.738                 & 0.631                & 0.927           & 0.980            \\
MVF-Net~\cite{MVF-Net}           & frame & 33.62 & 5.62 & 0.981            & 0.687                 & 0.599                & 0.927           & 0.971    \\
ResNet-50~\cite{he2016deep} & frame & 25.61 & 3.87 & 0.984 & 0.637 & 0.558 & 0.903 & 0.886 
\\ \midrule
EventNet~\cite{Eventnet}          & voxel  & 2.81 & 0.91 & 0.752            & 0.425                 & 0.171                & 0.750           & 0.833            \\
RG-CNNs~\cite{asl_dvs}           & voxel & 19.46 & 0.79 & 0.990            & 0.657                 & 0.540                & 0.914           & 0.901            \\
EV-VGCNN~\cite{EV-VGCNN}          & voxel & \textbf{0.84} & 0.70  & 0.994            & 0.748                 & 0.651                & 0.953           & 0.983            \\
VMV-GCN~\cite{xie2022vmv}          & voxel & 0.86 & 1.30 & 0.995            & 0.778                 & 0.663                & 0.932           & 0.989            \\
\midrule
Gabor-SNN~\cite{gabor_snn}         & spike & - & - & 0.837            & 0.196                 & 0.245                & 0.789           & -                \\
PLIF~\cite{PLIF}              & spike & 35.02 & 63.21 & 0.996            & -                     & 0.685                & -               & -                \\ \midrule
% Pointnet++~\cite{pointnet++}        & point-based   & 0.541            & 0.332                 & 0.148                & 0.544           & 0.575            \\
% Point Transformer~\cite{point_transformer} & point-based   & 0.998            & 0.642                 & 0.678                & 0.912           & \textbf{0.999}   \\ \midrule
\textbf{Ours}     & tensor  & 7.39 & \textbf{0.51} & \textbf{0.999}   & \textbf{0.789}        & \textbf{0.715}       & \textbf{0.954}       & \textbf{0.999} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}
\setlength{\tabcolsep}{1.4pt}

==> sections_full/tables/detection_results.tex <==
\setlength{\tabcolsep}{6pt}
\begin{table*}
\begin{center}
\caption{Comparison results for event-based object detection.}
\label{table:detection_results}
\begin{tabular}{lrcrrrrrr}
\toprule\noalign{\smallskip}
\multirow{2}{*}{\textbf{Methods}} & \multirow{2}{*}{\textbf{Representation}} & \multirow{2}{*}{\textbf{Async.}} & \multirow{2}{*}{\textbf{Parameters (M)}} & \multicolumn{2}{c}{\textbf{N-Caltech101}~\cite{n_caltech101}} & \multicolumn{2}{c}{\textbf{Gen1}~\cite{gen1}} \\
% \cmidrule{5-6} \cmidrule{7-8}
 & & & & mAP & MFLOP/ev & mAP & MFLOP/ev \\
\noalign{\smallskip}
\midrule
\noalign{\smallskip}
YOLE~\cite{yole} & frame & \Checkmark & - & 0.398 & 3682 & - & - \\
Asynet~\cite{asynet} & frame & \Checkmark & 133 & {\bf0.643} & 200 & 0.129 & 205 \\
\midrule
RED~\cite{1Mdetection} & voxel & \XSolidBrush & 24 & - & - & {\bf 0.40} & 4712 \\
NVS-S~\cite{nvs-s} & voxel & \Checkmark &  - & 0.346 & 7.8 & 0.086 & 7.8 \\
AEGNN~\cite{aegnn} & voxel & \Checkmark & - & 0.595 & \underline{0.37} & 0.163 & \underline{0.39} \\
\midrule
Spike-VGG~\cite{spike-detection} & spike & \Checkmark & 12.64 & - & - & 0.174 & 2.83 \\
Spike-MobileNet~\cite{spike-detection} & spike & \Checkmark & 24.26 & - & - & 0.147 & 1.11 \\
Spike-DenseNet~\cite{spike-detection} & spike & \Checkmark & 8.2 & - & - & 0.189 & 0.60 \\
\midrule
Ours & tensor & \Checkmark & - & \underline{0.619} & {\bf0.15} & \underline{0.218} & {\bf0.22} \\

\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> sections_full/tables/optical_flow_results.tex <==
\setlength{\tabcolsep}{5.1pt}
\begin{table*}
\begin{center}
\caption{Comparison results for event-based optical flow estimation. REP. and Async. are short for Representation and Asynchronous.}
\label{table:optical_flow_results}
\begin{tabular}{lrcrcccccccc}
\toprule\noalign{\smallskip}
\multirow{2}{*}{\textbf{Methods}} & \multirow{2}{*}{\textbf{REP.}} & \multirow{2}{*}{\textbf{Async.}} &\multirow{2}{*}{\textbf{FLOPs (G)}} & \multicolumn{2}{c}{\textbf{indoor\_flying1}} & \multicolumn{2}{c}{\textbf{indoor\_flying2}} & \multicolumn{2}{c}{\textbf{indoor\_flying3}} & \multicolumn{2}{c}{\textbf{outdoor\_day1}} \\
 & & & & AEE & OUT & AEE & OUT & AEE & OUT & AEE & OUT \\
\noalign{\smallskip}
\midrule
\noalign{\smallskip}
EvFlowNet~\cite{ev_flownet} & frame & \XSolidBrush & 24.37 & \underline{1.03} & 2.20 & \underline{1.72} & \underline{15.10} & 1.53 & 11.90 & \underline{0.49} & \underline{0.20} \\
FireNet~\cite{firenet} & frame & \XSolidBrush & 18.47 & 1.57 & 4.34 & 1.87 & 18.12 & 1.61 & 12.80 & 0.87 & 2.85 \\ \midrule
LIF-EvFlowNet~\cite{spike-evflownet} & spike & \Checkmark & 33.36 & 1.78 & 19.76 & 2.57 & 32.75 & 2.16 & 24.46 & 0.50 & 0.46 \\
LIF-FireNet~\cite{spike-evflownet} & spike & \Checkmark & \underline{9.08} & 1.04 & \textbf{1.78} & 1.77 & 15.22 & \underline{1.52} & \underline{9.58} & 0.92 & 1.83 \\ \midrule
Ours & tensor & \Checkmark & \textbf{3.58} & \textbf{1.01} & \underline{2.13} & \textbf{1.70} & \textbf{12.91} & \textbf{1.43} & \textbf{7.51} & \textbf{0.38} & \textbf{0.05} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> sections_short/figures/backbone.tex <==
\begin{figure*}[t]
\centering
\subfloat[Event Transformer Backbone]{\includegraphics[width=0.81\textwidth]{figures/backbone0.pdf}
\label{fig:et_backbone}}
\subfloat[Event Transformer Block]{\includegraphics[width=0.18\textwidth]{figures/backbone1.pdf}
\label{fig:et_block}}
\caption{{\bf Event Transformer.} \textbf{(a)} Five-stage backbone with $N\times4$ raw events input and $\frac{N}{128}\times(32C+4)$ output. For each event, output includes the original 4-channel attributes and aggregated features. 
For simplicity, we only give the size of features at each stage. \textbf{(b)} The Event Transformer Block (ETB) applies three-way  attentions in parallel for information aggregation. 
% \Salnote{Change \#Stage 1, 2  to Stage 1, 2  etc. in  (a)}
}
\label{fig:network}
\end{figure*}


==> sections_short/figures/cover.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=.32\textwidth]{figures/cover_0.pdf}
\label{fig:representation_forms}
\caption{\textbf{Different representations of the events.}}
\label{fig:representation_forms}
\end{figure}


==> sections_short/related_work.tex <==
\subsection{Event Representation Methods}
Given the popularity and prevalence of deep neural network (DNN) for 2D images, it is attractive to re-use them for event cameras. 
A straightforward approach is to convert event sequence into a 2D image by aggregating events in a preset time duration (e.g., \SI{33}{\milli\second}) into a gray-scale frame, as shown in Fig.~\ref{fig:representation_forms}. A number of such frame-based event representation approaches have been proposed in \cite{hfirst, hots, nCars, EST, AMAE, M-LSTM, MVF-Net, asynet, yole, ev_flownet, firenet}, but they introduces motion blur by discarding the fine time granularity in event cameras. 
An alternative approach is to convert events into a 3D point cloud and apply 3D DNNs for different tasks. 
Voxel-based representation~\cite{Eventnet, asl_dvs, EV-VGCNN, nvs-s, aegnn} converts events into a sequence of spatially-scattered 3D voxels by aggregating events in a relatively-short time duration.
Some methods~\cite{gabor_snn, PLIF, spike-evflownet} represent events as impulses, as demonstrated in Fig~\ref{fig:representation_forms}, which resemble spikes in human brain neurons and try to process them with the spiking neural network (SNN), 
Nevertheless, a spike in SNN is an impulse response function which is not differentiable. Thus, the inability of SNN to usegradient-based backpropagation and the need for specialized hardware implementation limit its applications. 

\subsection{Event-Based Vision}
Event cameras were first used in SLAM because of their low latency and bandwidth savings compared to conventional video cameras. In SLAM, the most common vision task is the detection of calibration plates and feature points. Therefore, several methods proposed to detect corners, lines, and edges by manually designing feature extractors \cite{corner_1,corner_2,corner_3}. As event cameras are upgraded and popularized, they are increasingly used in tasks such as object recognition~\cite{nMnist,n_caltech101,cifar10_dvs,nCars,asl_dvs} and detection~\cite{1Mdetection,n_caltech101}. Extracting semantic information from purely hand-designed features is extremely difficult; therefore, several methods have converted events into images to extract features with DNNs~\cite{ev_meet_dl,ev_flownet,hfirst,hots,EST,AMAE,M-LSTM,MVF-Net}. For instance, \cite{ev_meet_dl} stacks a period of events into a two-channel image based on their polarity, which causes a loss of temporal information and the event data converts into a long-exposure photograph. \cite{ev_flownet} adds two channels to record the timestamp of the last event. To take full advantage of the temporal information, \cite{nCars} encodes the latest events into time-surfaces, but it loses the spatial features. \cite{EST,M-LSTM} attempt to generate event frames by adaptive selection of events using learning approaches. It is worth noting that all frame-based methods require selection of a time window. A shorter window leads to insufficient accumulated data for downstream tasks, while a longer one causes motion blur and defeats the original purpose of high response rate from event cameras.

Several methods have been introduced to represent and exploit the spatio-temporal correlations in the event data by processing them as 3D points ~\cite{asl_dvs,EV-VGCNN}. For instance. \cite{asl_dvs,EV-VGCNN,aegnn} use graph convolution network (GCN) to learn the relationship between down-sampled events because event data are extremely sparse and dense convolutions can be computationally intensive. The time required to build the graph structure can even exceed the time required for the recognition task itself. Furthermore, these methods pre-process data by voxelizing events, which reduces the temporal granularity of the event data.

In addition to DNN and GNN, some methods \cite{gabor_snn, PLIF, spike-evflownet} have used spiking neural networks (SNN) for event data processing. The design of SNNs simulating human neural response and event cameras simulating retinal activation appear to be a nice combination. Nevertheless, the challenges of training SNNs and the need for special hardware prevents SNN from being used in real-life applications \cite{tavanaei2019deep}. 

In summary, the current methods for processing of events face problems in combining the spatial and temporal information and preserving the fine temporal granularity. In our method, we use the raw events data as input to ensure the lossless time precision. Inspired by recent NLP literature ~\cite{bert,xlnet,transformer-xl}, we use a transformer to extract temporal features and fuse temporal features with spatial features by sparse convolutions.

\subsection{Transformer}
Transformer architecture was recently proposed in \cite{attention_is_all_u_need} and applied to machine translation, which contains self-attention layers without any recurrent or convolution blocks. In recent years, transformer-based methods have achieved huge success in NLP~\cite{bert,xlnet,transformer-xl} and vision tasks~\cite{vit,swin}. Transformer-based backbones achieve better performance compared to the convolution-based backbones because of their ability to model information over long duration. Recently, \cite{neimark2021video} has used video transformer to successfully process spatio-temporal information in videos. 
Recently, \cite{event_transformer_frame,event_transformer_video} have a trial to introduce transformer~\cite{vit} into event data by stacking events into frame losing time granularity.   
The NLP transformers~\cite{attention_is_all_u_need,bert,xlnet,transformer-xl} cannot consider the spatial information of events data, the image transformers cannot handle the temporal relationships of events, and the video transformer~\cite{neimark2021video} needs to voxelize events where the sparsity of events would result in a lot of redundant computations.
% Most related to our work is the Point Transformer\cite{point_transformer}. It suggest that point clouds are sets with semantic information that are non-uniformly distributed in space and are well suited for establishing intrinsic connections using the attention mechanism. 
% \Salnote{What is the most relevant transformer work? Why don't we discuss this point transformer?} 



==> sections_short/tables/classification_dataset.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table}
\begin{center}
\caption{List of Event-based Classifiaction Datasets}
\label{table:cls_datasets_compare}
\begin{threeparttable}
\begin{tabular}{lrrrr}
\toprule\noalign{\smallskip}
\textbf{Dataset} & \textbf{Camera} & \textbf{Source}\tnote{$\dagger$} & \textbf{Classes} \\
\noalign{\smallskip}
\midrule
\noalign{\smallskip}
\nmnist~\cite{nMnist} & ATIS Lab Sensor & shake cam  & 10 \\
\ncaltech~\cite{n_caltech101} & ATIS Lab Sensor  & shake cam & 101 \\
\cifar~\cite{cifar10_dvs} & ATIS Lab Sensor & shake cam & 10 \\
\ncars~\cite{nCars} & Profhesee Gen1 & real move & 2 \\
\asl~\cite{asl_dvs} & DAVIS240c  & real move & 24 \\
\bottomrule
\end{tabular}
\begin{tablenotes}
    \footnotesize
    \item[$\dagger$] Source of generating events.
    % \item[$\ddagger$] Average duration of event stream.
    \end{tablenotes}
\end{threeparttable}
\end{center}
\end{table}


==> sections_short/tables/detection_results.tex <==
\setlength{\tabcolsep}{2.6pt}
\begin{table}\small
\begin{center}
\caption{Event-based object detection.}
\label{table:detection_results}
\begin{tabular}{lrrrrrr}
\toprule\noalign{\smallskip}
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{2}{c}{\textbf{N-Caltech101}~\cite{n_caltech101}} & & \multicolumn{2}{c}{\textbf{Gen1}~\cite{gen1}} \\
\cmidrule{2-3} 
\cmidrule{5-6}
 & mAP & MFLOPs/ev & & mAP & MFLOPs/ev \\
\noalign{\smallskip}
\midrule
\noalign{\smallskip}
\Frame YOLE~\cite{yole}                             & 39.8 & 3682 & & - & - \\
\Frame Asynet~\cite{asynet}                         & {\bf64.3} & 200 & & 12.9 & 205 \\
\midrule                
% \Voxel RED~\cite{1Mdetection}                       & - & - & {\bf 40.0} & 4712 \\
\Voxel NVS-S~\cite{nvs-s}                           & 34.6 & 7.8 & & 8.6 & 7.8 \\
\Voxel AEGNN~\cite{aegnn}                           & 59.5 & \underline{0.37} & & 16.3 & \underline{0.39} \\
\midrule
\Spike Spike-VGG~\cite{spike-detection}             & - & - & & 17.4 & 2.83 \\
\Spike Spike-MobileNet~\cite{spike-detection}       & - & - & & 14.7 & 1.11 \\
\Spike Spike-DenseNet~\cite{spike-detection}        & - & - & & \underline{18.9} & 0.60 \\
\midrule
\Tensor Ours                                        & {\bf 64.3} & {\bf0.15} & & {\bf 21.8} & {\bf0.22} \\
\bottomrule
\vspace{-1cm}
\end{tabular}
\end{center}
\end{table}

